Is Child-Directed Speech Effective Training Data for Language Models?

While high-performing language models are typically trained on hundreds of billions of words, human children become fluent language users with a much smaller amount of data. What are the features of the data they receive, and how do these features support language modeling objectives? To investigate this question, we train GPT-2 and RoBERTa models on 29M words of English child-directed speech and a new matched, synthetic dataset (TinyDialogues), comparing to OpenSubtitles, Wikipedia, and a heterogeneous blend of datasets from the BabyLM challenge. We evaluate the syntactic and semantic knowledge of these models using developmentally-inspired evaluations. Through pretraining experiments, we test whether the global developmental ordering or the local discourse ordering of children's training data supports high performance relative to other datasets. The local properties of the data affect model results, but surprisingly, global properties do not. Further, child language input is not uniquely valuable for training language models. These findings support the hypothesis that, rather than proceeding from better data, the child's learning algorithm is substantially more data-efficient than current language modeling techniques.

==> backup/appendices_backup.tex <==
\section{TinyDialogues: Dataset Collection Details \& Examples}
\label{appendix:TD_collection}

Here we discuss some further dataset collection details for TinyDialogues (TD), with examples of TD conversations in Table \ref{tab:TD_examples}.

%When prompting GPT-4, we emphasize that the conversation should be realistic, the child should be the central participant with most or all of the speech directed towards them, and that the vocabulary should be limited to that of which a child of the particular age can understand.
The specific GPT-4 model we use for collecting our entire dataset is \textit{gpt-4-1106-preview}, which is GPT-4 Turbo with training data up to Apr 2023. %\footnote{\url{https://platform.openai.com/docs/models/gpt-4-turbo-and-gpt-4}}
To increase the diversity of the generated conversations, when prompting GPT-4, we also specify the particular type of conversation (Table \ref{tab:TD_conversation_types}), the approximate length or number of turns (5 or 10),\footnote{GPT-4 had a tendency to generate longer conversations, around 10 and 20 turns instead, respectively.} other potential participants in the conversation (Table \ref{tab:TD_participants}), and certain words (one noun, one verb, and one adjective) sampled from Wordbank CDI \cite{frank2021variability} (ages 2 \& 5) and AoA \cite{Kuperman2012AgeofacquisitionRF} (ages 10 \& 15), cut off by the seeded age, that must be included in the conversation for content diversity. The list of potential participants and content words varied by age, e.g. a 15-year-old teenager would likely not talk regularly with a babysitter. We also collect some additional metadata: a list and description of all participants in the conversation, and a brief description of the context/setting. We only use the dialogue portions for our experiments. The GPT-4 prompt is below.

\textbf{GPT-4 Prompt: }\textit{Please construct a realistic, approximately \{5, 10\}-turn dialogue directly involving a \{2, 5, 10, 15\}-year-old \{toddler, child, teenager\}\footnote{\textit{toddler} is used for age 2, \textit{child} for ages 5 and 10, and \textit{teenager} for age 15.} as a participant. The \{toddler, child, teenager\} is the central participant in the dialogue, with most/all speech directed towards them. Hence, for this dialogue, please limit the vocabulary to that of which a typical \{2, 5, 10, 15\}-year-old \{toddler, child, teenager\} would understand. The dialogue should be \{type\}.\footnote{A random conversation type along with its explanation is sampled each time from the ones in Table \ref{tab:TD_conversation_types}.} The dialogue should use the verb `\{verb\}', the noun `\{noun\}', and the adjective `\{adjective\}'. Please include the following participants along with the child: \{participants\}.\footnote{If $turn = 5$, we randomly sample one additional participant from the corresponding list in Table \ref{tab:TD_participants}. For $turn = 10$, we randomly sample two additional participants.} Participant labels should be surrounded by double asterisks, i.e. `**participant**'. If there are several of the same type of participant (e.g. multiple friends or classmates), please label them distinctly, e.g. `**Friend 1**' and `**Friend 2**'. Please list and describe the participants after `PARTICIPANTS:', briefly describe the context/setting of the dialogue after `SETTING:', and present the dialogue itself after `DIALOGUE:'. The turns of the dialogue should be separated by `\escape{n}\escape{n}'. Remember, please ensure the dialogue is realistic, and one that would likely occur in the real world directly involving a \{2, 5, 10, 15\}-year-old \{toddler, child, teenager\}."
}

\begin{table*}[t]
\centering
\small
%\scalebox{0.9}{
%\resizebox{\textwidth}{!}{
%\begin{tabular}{cc}
%\begin{tabularx}{\textwidth}{|X|X|}
\begin{tabularx}{\textwidth}{p{0.5cm}|p{14.5cm}}
\toprule
% & \multicolumn{2}{c}{ImageNet} & NYUv2 - Depth & COCOStuff - Segmentation \\
\textbf{Age} & \textbf{Example}\\
\midrule
2 & **Babysitter**: Look, the pool is all empty. All gone! \escape{n}\escape{n} **Toddler**: Water all gone? \escape{n}\escape{n} **Babysitter**: Yes, all gone. We let the water out. It went down, down, down. \escape{n}\escape{n} **Toddler**: Why? \escape{n}\escape{n} **Babysitter**: So the pool can dry. We don't want it to get yucky. \escape{n}\escape{n} **Toddler**: Pool fall? \escape{n}\escape{n} **Babysitter**: No, the pool didn't fall. The water fell out when we opened the plug. \escape{n}\escape{n} **Toddler**: Plug? \escape{n}\escape{n} **Babysitter**: Yes, the plug is like a little stopper that keeps the water in. When we pull it, water comes out. \escape{n}\escape{n} **Toddler**: More water? \escape{n}\escape{n} **Babysitter**: Not now. We'll fill the pool again another day, okay? \escape{n}\escape{n} **Toddler**: Okay. Play ball? \escape{n}\escape{n} **Babysitter**: Sure, let's play ball now. The pool will be here when we're ready to fill it up again.\\
\midrule
5 & **Teacher**: "Alright, everyone, it's time to clean up! **Child**, can you please help me by putting the crayons back in the box?" \escape{n}\escape{n} **Child**: "Yes! I can do that. The box is empty so I'll fill it up!" \escape{n}\escape{n} **Teacher**: "Thank you, that's very helpful. Make sure the lids are on tight so they don't dry out." \escape{n}\escape{n} **Child**: "I did it! Look, they're all inside now." \escape{n}\escape{n} **Teacher**: "Great job! Now, **Classmate**, can you and **Child** go and put the books back on the shelf, please?" \escape{n}\escape{n} **Classmate**: "Can we go to play after?" \escape{n}\escape{n} **Teacher**: "Yes, as soon as our classroom is tidy, we can all go outside and play."  \escape{n}\escape{n} **Child**: "Come on, let's put the books away fast so we can go play!"  \escape{n}\escape{n} **Classmate**: "Okay, let's do it! Race you to the shelf!"  \escape{n}\escape{n} **Teacher**: "Be careful running, but I love the enthusiasm! Thank you both for helping."\\
\midrule
10 & **Dad**: "Once upon a time, in a faraway kingdom, there lived an earless rabbit who loved to make pancakes." \escape{n}\escape{n} **Child**: "An earless rabbit? How could he hear if he wanted to flip the batter?" \escape{n}\escape{n} **Dad**: "Well, you see, this rabbit had a special talent. He could feel the vibrations of the batter sizzling on the pan. When it was time to flip, he'd give it a perfect toss." \escape{n}\escape{n} **Child**: "That's so cool! Did the rabbit have any friends?" \escape{n}\escape{n} **Dad**: "Yes! His best friend was a turtle who loved to swim. One day, they decided to have a pancake picnic by the lake." \escape{n}\escape{n} **Child**: "Did they swim in the lake after eating pancakes?" \escape{n}\escape{n} **Dad**: "They sure did. The turtle taught the rabbit how to swim, and they had the best day splashing around until the sun set."\\
\midrule
15 & **Girlfriend**: Hey, so what's the plan for this history project video? \escape{n}\escape{n} **Teenager**: We need to make a mini-documentary about the industrial revolution. I was thinking we could start by showing how machines changed production, like how they used to churn butter by hand before. \escape{n}\escape{n} **Girlfriend**: Oh, cool idea! We could use that old butter churn in your grandma's attic for a visual. What role do you want me to play in the video? \escape{n}\escape{n} **Teenager**: Could you narrate the parts about the technological advancements? You're really good at explaining stuff. \escape{n}\escape{n} **Younger Sibling**: Can I help too? I want to be in the video! \escape{n}\escape{n} **Teenager**: Sure, you can help us set up the scenes. But no forcible taking over, okay? We need to work together as a team. \escape{n}\escape{n} **Younger Sibling**: I promise I'll be good! Can I churn the butter for the scene? \escape{n}\escape{n} **Teenager**: That's perfect! It'll look more authentic with you doing it. Let's get everything ready and start filming. Thanks for helping out, both of you.\\
\bottomrule
%\end{tabular}
%}
%}
\end{tabularx}
\caption{Examples of collected TinyDialogues conversations by seed age.}
\label{tab:TD_examples}
\end{table*}


\begin{table*}[t]
\centering
%\scalebox{0.9}{
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c}
\toprule
% & \multicolumn{2}{c}{ImageNet} & NYUv2 - Depth & COCOStuff - Segmentation \\
\textbf{Conversation Type} & \textbf{Explanation}\\
\midrule
Explanatory & It should involve explaining something(s) and potentially answering question(s).\\
Functional & It should involve attempting to get something(s) done or accomplishing particular goal(s).\\
Narrative & It should involve telling a story (real or fictional) or sharing/recounting an experience.\\
Argumentative & It should involve conflict(s) or disagreement(s) that lead to an argument.\\
& In most cases, the argument should be resolved, resulting in the \{child, toddler, teenager\} learning.\\
\bottomrule
\end{tabular}
}
%}
\caption{The four TinyDialogues conversation types along with their explanations.}
\label{tab:TD_conversation_types}
\end{table*}

\begin{table*}[t]
\centering
\small
%\scalebox{0.9}{
%\resizebox{\textwidth}{!}{
\begin{tabular}{c|c}
\toprule
% & \multicolumn{2}{c}{ImageNet} & NYUv2 - Depth & COCOStuff - Segmentation \\
\textbf{TD Seed Age} & \textbf{Potential Participants}\\
\midrule
2 & \{mom, dad, older sibling, babysitter\}\\
\midrule
5 & \{mom, dad, older sibling, younger sibling, teacher,\\
& friend, classmate, grandparent, babysitter, neighbor\}\\
\midrule
10 & \{mom, dad, older sibling, younger sibling, teacher,\\
& friend, classmate, grandparent, babysitter, neighbor\}\\
\midrule
15 & \{mom, dad, older sibling, younger sibling, teacher, friend, classmate, \\
& grandparent, neighbor, coach, tutor, boyfriend, girlfriend\}\\
\bottomrule
\end{tabular}
%}
%}
\caption{The list of other potential participants in each TinyDialogues conversation by seed age.}
\label{tab:TD_participants}
\end{table*}



\section{Data Format \& Preprocessing}
\label{appendix:data_preprocessing}

\textbf{CHILDES: } We noticed some duplicate utterances in CHILDES conversations and removed these to the best of our ability. We preprocessed the CHILDES data to match the format of the TD examples in Table \ref{tab:TD_examples}. See below for an example of part of a single training example for CHILDES. Double asterisks surround speaker labels, double newline tokens separate utterances, and an end-of-text token marks the end of the conversation. Hence, this format was consistent across all conversations in both CHILDES and TD datasets.

\textit{**CHI**: Are those your stars? \escape{n}\escape{n} **MOT**: Can you say star? \escape{n}\escape{n} **CHI**: Star. \escape{n}\escape{n} **CHI**: Look. \escape{n}\escape{n} **CHI**: Stars. \escape{n}\escape{n} **MOT**: Stars. See? Look, look at the yellow star, a golden star. <|endoftext|>}

\textbf{TinyDialogues:} One inconsistency in the collected TD data was that the speaker label for the target child varied across conversations and ages. For 2-year-olds, GPT-4 labeled the child \textit{toddler}, and 15-year-olds were labeled \textit{teenager}. This is likely due to our prompt as discussed in Appendix \ref{appendix:TD_collection}. Further, within the same age, sometimes the label also differed (e.g. \textit{Child}, \textit{5-year-old child}, \textit{5-year-old}). To align with CHILDES, which only used the speaker label CHI for every target child, and make Zorro evaluation consistent across the board (see Appendix \ref{appendix:zorro}), we converted several plausible target child speaker labels in our TD dataset (based on manual examination) to \textit{Child}. We also tried our best to correct any other issues in the GPT-4 outputs, including occasional inconsistencies with newlines and double newline tokens.

\textbf{BabyLM:} We concatenated the data across the BabyLM sub-datasets, then sampled approximately 29M words to match the amount of data in CHILDES and TD, while keeping the original distribution among its sub-datasets intact. We sampled in order (i.e. starting from the beginning of each sub-dataset), as several BabyLM examples (e.g. for Wikipedia) span multiple lines, and random sampling would have broken up individual examples and eliminated coherence. We do no further preprocessing to the BabyLM data and keep the format of the original sub-datasets. In particular, we do not add an <|endoftext|> token to the end of each example (like we do with CHILDES and TD) as it is unclear where each example ends.%, e.g. some Wikipedia examples span multiple lines.

The Python NLTK package's \textit{word\_tokenize} function was used as part of our statistics calculations (discussed in Appendix \ref{appendix:data_statistics}). The parameters for this function are: \textit{language} is `english' (default) and \textit{preserve\_line} is `False' (default) so line breaks are ignored. Specifically, it was used for calculating the number of unique words in Appendix \ref{appendix:data_statistics}. For consistency purposes, data processing and sampling, and other word-related statistics (e.g. total word count, avg. words per utterance) were done by simply splitting the text by space.



\section{Dataset Statistics}
\label{appendix:data_statistics}

\textbf{CHILDES} consists of $\approx$11k conversations over $\approx$29M words. The mean length of utterances is low, at only 3.85 words (minus speaker label), which is likely partially due to the skew in age, where $\approx$90\% of the data is for children ages 2-5 (see Figure \ref{fig:CHILDES_words_skew_graph}). CHILDES contains $\approx$74.5k unique words and $\approx$448 utterances (on avg.) per conversation.

\textbf{BabyLM} consists of $\approx$443k unique words in the $\approx$29M word subsample we take for our experiments. Individual example statistics are not available as some examples (e.g. Wikipedia) span multiple lines, and no end of example markers were given. More specific details and statistics about the dataset (including its sub-datasets) can be found in \citet{warstadt2023findings}, e.g. Table 1 in their paper.

\textbf{TinyDialogues} consists of $\approx$130k conversations across $\approx$29M words. There are $\approx$14 utterances (on avg.) per conversation, $\approx$96k unique words, and 13.42 words (on avg.) per utterance (minus speaker label). Since TD contains a uniform distribution across ages (including older ages), it is not surprising that the word diversity and average length of utterance are higher than CHILDES. Further, the average TD conversation is shorter than CHILDES, resulting in a higher number of individual conversations. More detailed statistics for TD (broken down by age) are in Table \ref{tab:TD_dataset_stats}. As expected, the vocabulary (unique words) and average length of utterance increase with age. Conversely, the total number of conversations and average utterances per conversation decrease with age.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.50\textwidth]{figures/CHILDES_words_graph_2.pdf}
    %\\\vspace{-0.2\abovedisplayskip}
    \caption{Total CHILDES word counts (utterances only, no metadata) by age.} \label{fig:CHILDES_words_skew_graph}
\end{figure}


\begin{table*}[t]
\centering
\small
%\scalebox{0.9}{
\begin{tabular}{cccccc}
\toprule
% & \multicolumn{2}{c}{ImageNet} & NYUv2 - Depth & COCOStuff - Segmentation \\
\textbf{Age} & \textbf{Conversations} & \textbf{Total Words} & \textbf{Unique Words} & \textbf{Avg. Utterances per Convo} & \textbf{Avg. Words per Utterance}\\
\midrule
2                 & 43,697 & 7,183,704 & 16,269 & 15.75 & 8.32\\
5                 & 33,248 & 7,194,902 & 15,534 & 14.01 & 13.36\\
10                & 27,198 & 7,196,356 & 42,508 & 13.61 & 17.35\\
15                & 25,589 & 7,199,752 & 73,484 & 12.88 & 19.77\\
Total             & 129,732 & 28,774,714 & 95,868 & 14.29 & 13.42\\
\bottomrule
\end{tabular}
%}
\caption{TinyDialogues dataset statistics broken down by seed age.}
\label{tab:TD_dataset_stats}
\end{table*}



\section{Further Training \& Compute Details}
\label{appendix:compute_details}

We searched through different values of the learning rate (LR) for GPT-2 training. Specifically, $LR = \{1e-06,5e-06,1e-05,5e-05,1e-04,5e-04,1e-03\}$. Through initial experiments, we found that $LR = 1e-04$ seemed to result in the best convergence behavior across the board, and used that for all our training experiments.

Our experiments were run on varying GPUs. This included a single RTX 3090TI (24GB VRAM), up to eight A40s (48GB VRAM each), up to eight A100s (80GB VRAM each), and up to four H100s (80GB VRAM each). Training time varied by the type and number of GPUs and the particular experiment (e.g. number of repeated buckets).


\section{Zorro Evaluation Details}
\label{appendix:zorro}

Zorro was inspired by BLiMP \cite{warstadt-etal-2020-blimp-benchmark} and is a modification for child-directed language (e.g. lower vocabulary). However, it was designed specifically for masked language models such as RoBERTa. To adapt it to GPT-2, we reformatted the Zorro data to match the BLiMP format and used the BLiMP evaluation in the BabyLM evaluation suite\footnote{\url{https://github.com/babylm/evaluation-pipeline-2023}} since the difference is mainly just the data. Further, we use the full Zorro test suite and do not filter examples by vocabulary. Hence, our results are not comparable to \citet{qin2024systematic} who filter Zorro examples by training vocabulary.

To better match the training data format and assess the effects of speaker labels, we came up with three variations of Zorro: 1) the original Zorro sentences (used to assess BabyLM), 2) the sentences with a common CHILDES speaker label prepended (used to assess CHILDES), and 3) the sentences with a common TD speaker label prepended (used to assess TD). To further match the training data as shown in Appendix \ref{appendix:data_preprocessing}, the speaker labels were surrounded by double asterisks, and sentences included double newline tokens (before and after). We used the mother speaker label (MOT) for CHILDES, and the child speaker label (Child) for TD (see Appendix \ref{appendix:data_preprocessing}), as these were some of the most frequent speaker labels for each dataset respectively (see Table \ref{tab:speaker_labels}). Further, preliminary experiments showed that these particular labels worked best for assessing each model.

\begin{table}[t]
\centering
\small
%\scalebox{0.9}{
\begin{tabular}{lccc}
\toprule
% & \multicolumn{2}{c}{ImageNet} & NYUv2 - Depth & COCOStuff - Segmentation \\
\textbf{Dataset} & \textbf{Speaker Label} & \textbf{Frequency} & \textbf{Proportion}\\
\midrule
CHILDES & MOT                 & 1,905,187 & 45.7\%\\
CHILDES & CHI                 & 1,593,073 & 38.2\%\\
CHILDES & INV                 & 188,712 & 4.5\%\\
CHILDES & FAT                 & 164,248 & 3.9\%\\
\midrule
TD & Child               & 735,176 & 46.6\%\\
TD & Mom                 & 132,746 & 8.4\%\\
TD & Dad                 & 129,568 & 8.2\%\\
TD & Older Sibling       & 120,468 & 7.6\%\\
\bottomrule
\end{tabular}
%}
\caption{List of the top speaker labels for CHILDES and TD training splits along with their frequencies and proportions. This is after converting all target child labels for TD to \textit{Child}, as described in Appendix \ref{appendix:data_preprocessing}. For CHILDES: MOT stands for \textit{mother}, CHI for \textit{child}, INV for \textit{investigator}, and FAT for \textit{father}.}
\label{tab:speaker_labels}
\end{table}



\section{Further Experimental Motivation}
\label{appendix:buckets_motivation}

If a dataset can be described as a concatenation of equal-sized buckets A, B, and C, the repeated bucket approach can be described as $An \ Bn \ Cn$. The inspiration for this approach is due to several reasons, other than being a compromise between standard iterated training and human learning (as discussed in Section \ref{sec:model_training}). Firstly, the iterative approach (training across the entire dataset several times) can potentially \textit{wash away} global ordering effects (especially when the epoch count is high) as global order differences mainly exist within each individual epoch. When trained across several epochs, its effects may be less noticeable. The repeated buckets approach maintains the global order across training as a whole. The model can learn more from each bucket before moving to the next. %Further, a way that children and humans use to learn language (and in general) is to revisit or repeat content at a certain level before moving up in difficulty. This allows us to ensure that we are sufficiently capable at a difficulty level before moving further. The RB approach is somewhat analogous to this.

\section{Further Experimental Results}
\label{appendix:results}

In addition to the experiments discussed in Section \ref{sec:results_and_analysis}, we tried different values of $n$ (number of times to repeat each bucket) for CHILDES and TD repeated buckets experiments. In particular, $n = 3, 5, 10, 20$. The chosen models for the repeated bucket experiments are the final models at the end of training. For CHILDES, we also tried different values of $b$ (number of buckets, or approximately equal sections to divide the dataset into) using the global age order. In particular, $b = 3, 5, 10$. We report average results for different values of $n$ and $b$ in Tables \ref{tab:eval_results_n} and \ref{tab:eval_results_b}, respectively. We also compare the typical iterative training approach (20 epochs) to repeated buckets using $n=20$ (analogous to 20 epochs). Results are in Table \ref{tab:eval_results_20-epochs}.

\begin{table}[t]
\centering
\small
%\scalebox{0.9}{
\begin{tabular}{lccc}
\toprule
% & \multicolumn{2}{c}{ImageNet} & NYUv2 - Depth & COCOStuff - Segmentation \\
\textbf{Model} & \textbf{$n$} & \textbf{Zorro} & \textbf{WS}\\
\midrule
CHILDES                 & 3 & 68.89\% & 0.10\\
CHILDES                 & 5 & 72.02\% & 0.14\\
CHILDES                 & 10 & 77.01\% & 0.19\\
CHILDES                 & 20 & 75.75\% & 0.23\\
\midrule
TD                 & 3 & 71.51\% & 0.18\\
TD                 & 5 & 74.48\% & 0.23\\
TD                 & 10 & 79.21\% & 0.32\\
TD                 & 20 & 79.65\% & 0.41\\
\bottomrule
\end{tabular}
%}
\caption{Evaluation results of our GPT-2 models, comparing different values of $n$, broken down by dataset. These results are averaged across three different global ordering methods: age order, reverse order, and random order. For CHILDES, we use $b=5$.}
\label{tab:eval_results_n}
\end{table}

\begin{table}[t]
\centering
\small
%\scalebox{0.9}{
\begin{tabular}{lccc}
\toprule
% & \multicolumn{2}{c}{ImageNet} & NYUv2 - Depth & COCOStuff - Segmentation \\
\textbf{Model} & \textbf{$b$} & \textbf{Zorro} & \textbf{WS}\\
\midrule
CHILDES                 & 3 & 73.36\% & 0.35\\
CHILDES                 & 5 & 72.12\% & 0.35\\
CHILDES                 & 10 & 70.06\% & 0.35\\
\bottomrule
\end{tabular}
%}
\caption{Evaluation results of our CHILDES GPT-2 models, comparing different values of $b$. These results are averaged across three experiments each: global age order with $n=3,5,10$.}
\label{tab:eval_results_b}
\end{table}

\begin{table}[t]
\centering
\small
%\scalebox{0.9}{
\begin{tabular}{lccc}
\toprule
% & \multicolumn{2}{c}{ImageNet} & NYUv2 - Depth & COCOStuff - Segmentation \\
\textbf{Model} & \textbf{Approach} & \textbf{Zorro} & \textbf{WS}\\
\midrule
CHILDES                 & 20-epochs & 77.13\% & 0.52\\
CHILDES                 & $b=5,n=20$ & 75.75\% & 0.48\\
\midrule
TD                 & 20-epochs & 79.41\% & 0.54\\
TD                 & $n=20$ & 79.65\% & 0.54\\
\bottomrule
\end{tabular}
%}
\caption{Evaluation results of our GPT-2 models, comparing typical iterative training (20 epochs) vs. repeated buckets with $n=20$ (and $b=5$ for CHILDES), broken down by dataset. These results are averaged across three experiments each: the three different global ordering methods (age order, reverse order, random order).}
\label{tab:eval_results_20-epochs}
\end{table}


\section{Importance of Speaker Labels}
\label{appendix:speaker_labels}

As an additional experiment, we also assess the importance of having speaker labels for each utterance. We train some versions of our models after removing all speaker labels (including their surrounding double asterisks). The results are reported in Table \ref{tab:eval_results_speaker-labels}. As seen, removing speaker labels greatly detriments syntax and grammar learning (Zorro), but semantics (WS) appears unaffected.

\begin{table}[t]
\centering
\small
%\scalebox{0.9}{
\begin{tabular}{lccc}
\toprule
% & \multicolumn{2}{c}{ImageNet} & NYUv2 - Depth & COCOStuff - Segmentation \\
\textbf{Model} & \textbf{Speaker Label?} & \textbf{Zorro} & \textbf{WS}\\
\midrule
CHILDES                 & Yes & 77.65\% & 0.21\\
CHILDES                 & No & 71.84\% & 0.22\\
\midrule
TD                 & Yes & 80.67\% & 0.37\\
TD                 & No & 76.53\% & 0.37\\
\bottomrule
\end{tabular}
%}
\caption{Evaluation results of our GPT-2 models, comparing speaker label vs. no speaker label for conversation utterances, broken down by dataset. These results are averaged across two experiments each: global random order with the typical iterative approach (20 epochs) and $n=10$ (with $b=5$ for CHILDES).}
\label{tab:eval_results_speaker-labels}
\end{table}



\section{Convergence Behavior of Models}
\label{appendix:convergence_behavior}

We plot the convergence graphs (train and validation losses vs. epoch) for several sets of our experiments in Figures \ref{fig:dataset_convergence_graphs} to \ref{fig:micro_intervention_convergence_graphs}. For the repeated buckets experiments, we treat the entire training run as a single epoch. We can notice interesting patterns/trends in the convergence behavior of models depending on several factors including the global ordering and curricularization method. 

From Figure \ref{fig:dataset_convergence_graphs}, we see that BabyLM converges to higher losses than CHILDES and TD, although it seems to perform better at test-time for syntax and semantics (as discussed in Section \ref{sec:results_and_analysis}). Losses during training could simply be higher as the dataset is more complicated and varied since it is a mixture.

From Figure \ref{fig:TD_20-epoch_convergence_graphs}, we can see that when we train using the typical iterative epochs approach, the training loss has a cyclical pattern using global age order and reverse order, while it converges smoothly for random order. From Figures \ref{fig:CHILDES_global_order_10n_convergence_graphs} and \ref{fig:TD_global_order_10n_convergence_graphs}, we see that when using the repeated buckets approach for both CHILDES and TD, global age order leads to a slowly cyclical increase in the training loss, while it generally decreases for reverse and random order. Throughout these experiments, while the training loss differs and individual buckets exhibit differing patterns, the high-level behavior of the validation loss and hence overall learning is similar. This aligns with the results we saw in Section \ref{sec:results_and_analysis}.

From Figures \ref{fig:bucket_convergence_graphs_by_n} and \ref{fig:bucket_convergence_graphs_by_b}, we see that varying $b$ and $n$ result in minor changes in behavior for the training loss. Specifically, by increasing $n$, the training loss has a more clearly defined cyclical pattern, and the losses converge to lower values. This is expected, since increasing $n$ is analogous to training on more epochs. From Figure \ref{fig:micro_intervention_convergence_graphs}, we see that local interventions -- randomly shuffling utterances and removing speaker labels (see Appendix \ref{appendix:speaker_labels}) -- have minor effects on convergence behavior.

%Convergence graphs and analysis

\section{Licenses and Intended Use}
\label{appendix:licenses}

We used all existing datasets and models for their intended use. GPT-2 is licensed under the Modified MIT License. CHILDES is made available under TalkBank which is governed by the Creative Commons CC BY-NC-SA 3.0 copyright license (see \url{https://talkbank.org/share/rules.html}). We plan to release the TinyDialogues dataset under the standard MIT license. Information about the BabyLM challenge and its dataset (which is a collection of portions of several sub-datasets) is at \url{https://babylm.github.io/index.html}.


\section{Code \& Data}
\label{appendix:code_and_data}

We plan to publicly release all our code and data. Some of the code was written with the assistance of ChatGPT (specifically, GPT-4 and GPT-4o).


\begin{figure}[t]
%\vspace{-8mm}
    \centering
    %\hspace*{-0.63cm} % Adjust this value as needed to align the figures to the left
    \hspace*{-0.75cm}
    \includegraphics[width=0.57\textwidth]{figures/datasets/GPT2-small_CHILDES_randomized_ABC_20-epochs_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/datasets/GPT2-small_tinydialogue_randomized_ABC_20-epochs_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/datasets/GPT2-small_babyLM_20M_1e-04_20-epochs_trainer_state.json_loss_curves.png}
    \caption{Convergence graphs (train and val loss) by dataset, using iterative training for 20 epochs. From top to bottom: CHILDES, TinyDialogues, BabyLM.} \label{fig:dataset_convergence_graphs}
\end{figure}

\begin{figure}[t]
    \centering
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/TD/20_epoch/GPT2-small_tinydialogue_ordered_ABC_20-epochs_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/TD/20_epoch/GPT2-small_tinydialogue_reversed_ABC_20-epochs_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/TD/20_epoch/GPT2-small_tinydialogue_randomized_ABC_20-epochs_trainer_state.json_loss_curves.png}
    \caption{Convergence graphs (train and val loss) of TinyDialogues using the typical iterative training approach for 20 epochs, for different global orders. From top to bottom: age order, reverse order, random order.} \label{fig:TD_20-epoch_convergence_graphs}
\end{figure}

\begin{figure}[t]
    \centering
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/10n/GPT2-small_CHILDES_ordered_5b_10n_1e-04_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/10n/GPT2-small_CHILDES_reversed_5b_10n_1e-04_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/10n/GPT2-small_CHILDES_randomized_5b_10n_1e-04_trainer_state.json_loss_curves.png}
    \caption{Convergence graphs (train and val loss) of CHILDES using the repeated buckets training approach with $b=5, n=10$, for different global orders. From top to bottom: age order, reverse order, random order.} \label{fig:CHILDES_global_order_10n_convergence_graphs}
\end{figure}

\begin{figure}[t]
    \centering
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/TD/10n/GPT2-small_tinydialogue_ordered_10n_1e-04_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/TD/10n/GPT2-small_tinydialogue_reversed_10n_1e-04_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/TD/10n/GPT2-small_tinydialogue_randomized_10n_1e-04_trainer_state.json_loss_curves.png}
    \caption{Convergence graphs (train and val loss) of TinyDialogues using the repeated buckets training approach with $n=10$, for different global orders. From top to bottom: age order, reverse order, random order.} \label{fig:TD_global_order_10n_convergence_graphs}
\end{figure}

\begin{figure}[t]
    \centering
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/buckets_n/GPT2-small_CHILDES_ordered_5b_3n_1e-04_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/buckets_n/GPT2-small_CHILDES_ordered_5b_5n_1e-04_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/buckets_n/GPT2-small_CHILDES_ordered_5b_10n_1e-04_trainer_state.json_loss_curves.png}
    \hspace*{-0.65cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.56\textwidth]{figures/CHILDES/buckets_n/GPT2-small_CHILDES_ordered_5b_20n_1e-04_trainer_state.json_loss_curves.png}
    \caption{Convergence graphs (train and val loss) of CHILDES using the repeated buckets training approach with $b=5$, for different values of $n$. From top to bottom: $n=3,5,10,20$.} \label{fig:bucket_convergence_graphs_by_n}
\end{figure}

\begin{figure}[t]
    \centering
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/buckets_b/GPT2-small_CHILDES_ordered_3b_5n_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/buckets_b/GPT2-small_CHILDES_ordered_5b_5n_loss_curves.png}
    \hspace*{-0.75cm} % Adjust this value as needed to align the figures to the left
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/buckets_b/GPT2-small_CHILDES_ordered_10b_5n_loss_curves.png}
    \caption{Convergence graphs (train and val loss) of CHILDES using the repeated buckets training approach with $n=5$, for different values of $b$. From top to bottom: $b=3,5,10$.} \label{fig:bucket_convergence_graphs_by_b}
\end{figure}

\begin{figure}[t]
    \centering
    \hspace*{-0.75cm}
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/micro/GPT2-small_CHILDES_randomized_5b_10n_1e-04_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm}
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/micro/GPT2-small_CHILDES_randomized_5b_10n_utterances-randomized_1e-04_trainer_state.json_loss_curves.png}
    \hspace*{-0.75cm}
    \includegraphics[width=0.57\textwidth]{figures/CHILDES/micro/GPT2-small_CHILDES_randomized_5b_10n_no-speaker-labels_1e-04_trainer_state.json_loss_curves.png}
    \caption{Convergence graphs (train and val loss) of CHILDES, looking at the effects of local interventions -- shuffling utterances and removing speaker labels -- using global random ordering with the repeated buckets approach ($b=5,n=10$). From top to bottom: original data (no changes), random shuffling of utterances, no speaker labels for utterances.} \label{fig:micro_intervention_convergence_graphs}
\end{figure}

%CHILDES dataset
%GPT-2 model
%Zorro Eval
%WS Eval
